Learning Weighted Finite Automata over the Max-Plus Semiring and its Termination

Active learning of finite automata has been vigorously pursued for the purposes of analysis and explanation of black-box systems. In this paper, we study an L*-style learning algorithm for weighted automata over the max-plus semiring. The max-plus setting exposes a "consistency" issue in the previously studied semiring-generic extension of L*: we show that it can fail to maintain consistency of tables, and can thus make equivalence queries on obviously wrong hypothesis automata. We present a theoretical fix by a mathematically clean notion of column-closedness. We also present a nontrivial and reasonably broad class of weighted languages over the max-plus semiring in which our algorithm terminates.

==> data/automata_size.tikz.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.4p0 (Lua 5.4; terminal rev. Jun 2020, script rev. 114)
%% 2020年09月10日 19時07分53秒
\tikzset{every node/.append style={font={\fontsize{16.0pt}{19.2pt}\selectfont}}}
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.816,1.577)--(1.996,1.577);
\draw[gp path] (11.617,1.577)--(11.437,1.577);
\node[gp node right] at (1.522,1.577) {$0$};
\draw[gp path] (1.816,2.155)--(1.996,2.155);
\draw[gp path] (11.617,2.155)--(11.437,2.155);
\node[gp node right] at (1.522,2.155) {$10$};
\draw[gp path] (1.816,2.733)--(1.996,2.733);
\draw[gp path] (11.617,2.733)--(11.437,2.733);
\node[gp node right] at (1.522,2.733) {$20$};
\draw[gp path] (1.816,3.310)--(1.996,3.310);
\draw[gp path] (11.617,3.310)--(11.437,3.310);
\node[gp node right] at (1.522,3.310) {$30$};
\draw[gp path] (1.816,3.888)--(1.996,3.888);
\draw[gp path] (11.617,3.888)--(11.437,3.888);
\node[gp node right] at (1.522,3.888) {$40$};
\draw[gp path] (1.816,4.466)--(1.996,4.466);
\draw[gp path] (11.617,4.466)--(11.437,4.466);
\node[gp node right] at (1.522,4.466) {$50$};
\draw[gp path] (1.816,5.044)--(1.996,5.044);
\draw[gp path] (11.617,5.044)--(11.437,5.044);
\node[gp node right] at (1.522,5.044) {$60$};
\draw[gp path] (1.816,5.621)--(1.996,5.621);
\draw[gp path] (11.617,5.621)--(11.437,5.621);
\node[gp node right] at (1.522,5.621) {$70$};
\draw[gp path] (1.816,6.199)--(1.996,6.199);
\draw[gp path] (11.617,6.199)--(11.437,6.199);
\node[gp node right] at (1.522,6.199) {$80$};
\draw[gp path] (1.816,6.777)--(1.996,6.777);
\draw[gp path] (11.617,6.777)--(11.437,6.777);
\node[gp node right] at (1.522,6.777) {$90$};
\draw[gp path] (1.816,1.577)--(1.816,1.757);
\draw[gp path] (1.816,6.777)--(1.816,6.597);
\node[gp node center] at (1.816,1.084) {$10$};
\draw[gp path] (3.041,1.577)--(3.041,1.757);
\draw[gp path] (3.041,6.777)--(3.041,6.597);
\node[gp node center] at (3.041,1.084) {$15$};
\draw[gp path] (4.266,1.577)--(4.266,1.757);
\draw[gp path] (4.266,6.777)--(4.266,6.597);
\node[gp node center] at (4.266,1.084) {$20$};
\draw[gp path] (5.491,1.577)--(5.491,1.757);
\draw[gp path] (5.491,6.777)--(5.491,6.597);
\node[gp node center] at (5.491,1.084) {$25$};
\draw[gp path] (6.717,1.577)--(6.717,1.757);
\draw[gp path] (6.717,6.777)--(6.717,6.597);
\node[gp node center] at (6.717,1.084) {$30$};
\draw[gp path] (7.942,1.577)--(7.942,1.757);
\draw[gp path] (7.942,6.777)--(7.942,6.597);
\node[gp node center] at (7.942,1.084) {$35$};
\draw[gp path] (9.167,1.577)--(9.167,1.757);
\draw[gp path] (9.167,6.777)--(9.167,6.597);
\node[gp node center] at (9.167,1.084) {$40$};
\draw[gp path] (10.392,1.577)--(10.392,1.757);
\draw[gp path] (10.392,6.777)--(10.392,6.597);
\node[gp node center] at (10.392,1.084) {$45$};
\draw[gp path] (11.617,1.577)--(11.617,1.757);
\draw[gp path] (11.617,6.777)--(11.617,6.597);
\node[gp node center] at (11.617,1.084) {$50$};
\draw[gp path] (1.816,6.777)--(1.816,1.577)--(11.617,1.577)--(11.617,6.777)--cycle;
\node[gp node center,rotate=-270] at (0.467,4.177) {Size of the learned WFA $\Aout$};
\node[gp node center] at (6.716,0.345) {Size of the target WFA $\Ain$};
\node[gp node left] at (2.600,8.323) {tol=0.5, $\rmax$\hspace{1em}};
\gpcolor{rgb color={0.580,0.000,0.827}}
\gpsetlinewidth{6.00}
\draw[gp path] (1.538,8.323)--(2.306,8.323);
\draw[gp path] (1.816,2.381)--(3.041,3.137)--(4.266,3.930)--(11.617,6.777);
\gpsetpointsize{8.00}
\gp3point{gp mark 5}{}{(1.816,2.381)}
\gp3point{gp mark 5}{}{(3.041,3.137)}
\gp3point{gp mark 5}{}{(4.266,3.930)}
\gp3point{gp mark 5}{}{(11.617,6.777)}
\gp3point{gp mark 5}{}{(1.922,8.323)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (2.600,7.830) {tol=1.0, $\rmax$};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.538,7.830)--(2.306,7.830);
\draw[gp path] (1.816,2.080)--(3.041,2.284)--(4.266,2.465)--(11.617,2.357);
\gp3point{gp mark 7}{}{(1.816,2.080)}
\gp3point{gp mark 7}{}{(3.041,2.284)}
\gp3point{gp mark 7}{}{(4.266,2.465)}
\gp3point{gp mark 7}{}{(11.617,2.357)}
\gp3point{gp mark 7}{}{(1.922,7.830)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (2.600,7.337) {tol=2.0, $\rmax$};
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (1.538,7.337)--(2.306,7.337);
\draw[gp path] (1.816,1.659)--(3.041,1.645)--(4.266,1.660)--(11.617,1.664);
\gp3point{gp mark 3}{}{(1.816,1.659)}
\gp3point{gp mark 3}{}{(3.041,1.645)}
\gp3point{gp mark 3}{}{(4.266,1.660)}
\gp3point{gp mark 3}{}{(11.617,1.664)}
\gp3point{gp mark 3}{}{(1.922,7.337)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (8.072,8.323) {tol=0.5, $\real$};
\gpcolor{rgb color={0.902,0.624,0.000}}
\draw[gp path] (7.010,8.323)--(7.778,8.323);
\draw[gp path] (1.816,3.017)--(3.041,3.970)--(4.266,4.945)--(11.617,5.787);
\gp3point{gp mark 4}{}{(1.816,3.017)}
\gp3point{gp mark 4}{}{(3.041,3.970)}
\gp3point{gp mark 4}{}{(4.266,4.945)}
\gp3point{gp mark 4}{}{(11.617,5.787)}
\gp3point{gp mark 4}{}{(7.394,8.323)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (8.072,7.830) {tol=1.0, $\real$};
\gpcolor{rgb color={0.941,0.894,0.259}}
\draw[gp path] (7.010,7.830)--(7.778,7.830);
\draw[gp path] (1.816,2.305)--(3.041,2.477)--(4.266,2.669)--(11.617,3.753);
\gp3point{gp mark 6}{}{(1.816,2.305)}
\gp3point{gp mark 6}{}{(3.041,2.477)}
\gp3point{gp mark 6}{}{(4.266,2.669)}
\gp3point{gp mark 6}{}{(11.617,3.753)}
\gp3point{gp mark 6}{}{(7.394,7.830)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (8.072,7.337) {tol=2.0, $\real$};
\gpcolor{rgb color={0.000,0.447,0.698}}
\draw[gp path] (7.010,7.337)--(7.778,7.337);
\draw[gp path] (1.816,1.973)--(3.041,2.006)--(4.266,2.068)--(11.617,2.148);
\gp3point{gp mark 2}{}{(1.816,1.973)}
\gp3point{gp mark 2}{}{(3.041,2.006)}
\gp3point{gp mark 2}{}{(4.266,2.068)}
\gp3point{gp mark 2}{}{(11.617,2.148)}
\gp3point{gp mark 2}{}{(7.394,7.337)}
\gpcolor{color=gp lt color border}
\gpsetlinewidth{1.00}
\draw[gp path] (1.816,6.777)--(1.816,1.577)--(11.617,1.577)--(11.617,6.777)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.816cm}{1.577cm}}{\pgfpoint{11.617cm}{6.777cm}}
\end{tikzpicture}
%% gnuplot variables


==> data/bell_table.tabular.tex <==
\begin{tabular}{ c | c c c | c c c | c c c }
\multirow{3}{*}{$(|\Sigma|, |A_{\mathrm{in}}|, \mathtt{tol})$} & \multicolumn{3}{c|}{succ. rate} & \multicolumn{3}{c|}{RMSE} & \multicolumn{3}{c}{$|A_{\mathrm{out}}|$} \\ \cline{2-10} 
 & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$} & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$} & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$}\\ 
 & minimized & not minimized &  & minimized & not minimized &  & minimized & not minimized & \\ \hline 
(5, 10, 0.5) & 1.0 & 1.0  & 1.0 & (6.42e-01,3.65e-02) & (5.85e-01,7.64e-02) & (5.37e-01,6.85e-02) & \tbcolor\bf (10.6,1.7) & (17.8,2.3) & (18.6,2.4) \\
(10, 10, 0.5) & 0.6 & 1.0  & 1.0 & (6.33e-01,6.19e-02) & (6.39e-01,5.09e-02) & (6.15e-01,3.37e-02) & \tbcolor\bf (15.7,1.2) & (32.2,8.5) & (22.0,2.8) \\
(20, 10, 0.5) & 0.2 & 1.0  & 1.0 & (7.23e-01,0.00e+00) & (5.39e-01,1.03e-01) & (6.12e-01,5.08e-02) & \tbcolor\bf (17.0,0.0) & (48.2,6.9) & (25.8,3.2) \\
(30, 10, 0.5) & 0.4 & 1.0  & 1.0 & (6.49e-01,2.77e-02) & (5.34e-01,6.15e-02) & (6.32e-01,3.23e-02) & \tbcolor\bf (21.0,4.0) & (66.2,8.6) & (29.2,2.3) \\
(5, 15, 0.5) & 1.0 & 1.0  & 1.0 & (6.71e-01,7.60e-02) & (5.91e-01,6.53e-02) & (5.67e-01,7.02e-02) & \tbcolor\bf (15.2,2.9) & (26.0,7.8) & (18.8,1.3) \\
(10, 15, 0.5) & 0.8 & 1.0  & 1.0 & (6.82e-01,3.96e-02) & (5.93e-01,6.58e-02) & (6.09e-01,5.81e-02) & \tbcolor\bf (28.5,6.5) & (63.0,10.2) & (31.2,3.3) \\
(20, 15, 0.5) & 0.4 & 1.0  & 1.0 & (7.18e-01,1.40e-02) & (5.55e-01,2.42e-02) & (6.24e-01,4.66e-02) & \tbcolor\bf (41.0,1.0) & (112.4,11.5) & (42.6,6.5) \\
(30, 15, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.42e-01,3.41e-02) & N/A & N/A & \tbcolor\bf (47.0,2.8) \\
(5, 20, 0.5) & 0.6 & 1.0  & 1.0 & (6.47e-01,4.75e-02) & (6.02e-01,8.48e-02) & (5.62e-01,5.33e-02) & (29.7,3.7) & (42.8,7.7) & \tbcolor\bf (26.0,3.0) \\
(10, 20, 0.5) & 0.8 & 1.0  & 1.0 & (6.50e-01,2.65e-02) & (5.91e-01,4.34e-02) & (6.26e-01,3.65e-02) & (48.8,5.1) & (109.8,13.4) & \tbcolor\bf (39.4,2.9) \\
(20, 20, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.46e-01,1.43e-02) & N/A & N/A & \tbcolor\bf (53.6,8.1) \\
(30, 20, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.43e-01,2.62e-02) & N/A & N/A & \tbcolor\bf (63.4,9.8) \\
(5, 50, 0.5) & 0.4 & 0.4  & 1.0 & (5.80e-01,1.97e-02) & (5.66e-01,9.04e-03) & (6.69e-01,3.97e-02) & (90.0,1.0) & (164.5,3.5) & \tbcolor\bf (44.8,12.5) \\
(10, 50, 0.5) & 0.4 & 0.0  & 1.0 & (1.07e+01,2.53e+00) & N/A & (6.71e-01,4.19e-02) & \tbcolor\bf (1.0,0.0) & N/A & (87.2,9.7) \\
(20, 50, 0.5) & 0.0 & 0.0  & 0.0 & N/A & N/A & N/A & N/A & N/A & N/A \\
(30, 50, 0.5) & 0.0 & 0.0  & 0.0 & N/A & N/A & N/A & N/A & N/A & N/A \\
(5, 10, 1.0) & 0.0 & 0.2  & 1.0 & N/A & (9.98e-01,0.00e+00) & (8.88e-01,1.24e-01) & N/A & \tbcolor\bf (8.0,0.0) & (10.0,1.1) \\
(10, 10, 1.0) & 0.4 & 0.8  & 1.0 & (8.92e-01,9.32e-02) & (9.32e-01,1.04e-01) & (8.37e-01,6.21e-02) & \tbcolor\bf (8.5,0.5) & (9.2,3.6) & (12.6,1.9) \\
(20, 10, 1.0) & 0.8 & 1.0  & 1.0 & (9.26e-01,4.67e-02) & (9.02e-01,3.85e-02) & (8.45e-01,1.06e-01) & \tbcolor\bf (9.0,0.7) & (9.6,3.0) & (12.8,3.3) \\
(30, 10, 1.0) & 0.6 & 1.0  & 1.0 & (8.93e-01,3.10e-02) & (9.51e-01,9.20e-02) & (7.99e-01,5.14e-02) & \tbcolor\bf (9.7,0.5) & (10.8,1.6) & (14.6,0.8) \\
(5, 15, 1.0) & 0.6 & 1.0  & 1.0 & (8.96e-01,1.38e-02) & (9.09e-01,7.80e-02) & (8.17e-01,1.44e-01) & \tbcolor\bf (2.3,0.5) & (5.2,2.5) & (9.2,1.8) \\
(10, 15, 1.0) & 0.6 & 0.6  & 1.0 & (9.27e-01,7.90e-02) & (1.00e+00,1.36e-02) & (8.41e-01,1.06e-01) & (12.0,2.2) & \tbcolor\bf (6.7,3.1) & (12.2,1.9) \\
(20, 15, 1.0) & 0.8 & 1.0  & 1.0 & (9.19e-01,5.59e-02) & (8.67e-01,9.07e-02) & (8.38e-01,4.01e-02) & \tbcolor\bf (15.0,0.7) & (16.4,3.5) & (15.8,0.4) \\
(30, 15, 1.0) & 0.4 & 0.8  & 1.0 & (8.98e-01,2.95e-02) & (9.24e-01,4.34e-02) & (8.68e-01,8.10e-02) & \tbcolor\bf (15.5,0.5) & (18.5,2.2) & (17.4,1.7) \\
(5, 20, 1.0) & 0.8 & 1.0  & 1.0 & (9.61e-01,1.22e-02) & (9.41e-01,6.14e-02) & (8.31e-01,5.62e-02) & (5.0,4.7) & \tbcolor\bf (4.2,2.6) & (11.4,1.4) \\
(10, 20, 1.0) & 0.6 & 0.6  & 1.0 & (9.71e-01,4.13e-02) & (9.40e-01,8.19e-02) & (8.53e-01,1.22e-01) & (15.3,4.5) & (16.7,2.6) & \tbcolor\bf (13.6,1.5) \\
(20, 20, 1.0) & 0.8 & 0.8  & 1.0 & (9.68e-01,5.14e-02) & (9.87e-01,5.91e-02) & (9.14e-01,2.35e-02) & \tbcolor\bf (16.2,5.4) & (17.0,8.3) & (18.4,1.9) \\
(30, 20, 1.0) & 0.6 & 1.0  & 1.0 & (9.53e-01,5.21e-02) & (9.64e-01,5.44e-02) & (9.30e-01,5.34e-02) & (20.0,0.8) & (28.2,5.9) & \tbcolor\bf (19.6,2.8) \\
(5, 50, 1.0) & 0.6 & 1.0  & 1.0 & (9.36e-01,6.51e-02) & (9.07e-01,7.83e-02) & (8.48e-01,9.69e-02) & \tbcolor\bf (3.7,1.2) & (5.6,3.9) & (13.0,3.0) \\
(10, 50, 1.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (9.33e-01,2.34e-02) & N/A & N/A & \tbcolor\bf (16.0,2.1) \\
(20, 50, 1.0) & 0.2 & 0.8  & 1.0 & (9.30e-01,0.00e+00) & (9.17e-01,4.48e-02) & (8.61e-01,9.75e-02) & (43.0,0.0) & (50.2,25.2) & \tbcolor\bf (25.0,5.6) \\
(30, 50, 1.0) & 0.0 & 0.8  & 1.0 & N/A & (8.69e-01,4.25e-02) & (8.87e-01,7.06e-02) & N/A & (60.2,30.4) & \tbcolor\bf (22.2,5.8) \\
(5, 10, 2.0) & 0.4 & 0.2  & 1.0 & (1.33e+00,6.76e-02) & (1.26e+00,0.00e+00) & (3.48e+00,3.06e+00) & (1.5,0.5) & \tbcolor\bf (1.0,0.0) & (5.8,1.9) \\
(10, 10, 2.0) & 0.6 & 0.6  & 0.6 & (1.27e+00,5.82e-02) & (1.27e+00,5.82e-02) & (1.14e+00,1.98e-01) & \tbcolor\bf (1.3,0.5) & \tbcolor\bf (1.3,0.5) & (5.7,0.5) \\
(20, 10, 2.0) & 0.2 & 0.2  & 1.0 & (1.25e+00,0.00e+00) & (1.25e+00,0.00e+00) & (1.21e+00,1.16e-01) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (7.4,1.7) \\
(30, 10, 2.0) & 0.6 & 0.4  & 1.0 & (1.33e+00,1.34e-02) & (1.33e+00,1.64e-02) & (1.26e+00,7.60e-02) & \tbcolor\bf (2.0,0.0) & \tbcolor\bf (2.0,0.0) & (6.6,0.5) \\
(5, 15, 2.0) & 0.8 & 0.8  & 0.8 & (1.18e+00,1.26e-01) & (1.18e+00,1.26e-01) & (2.87e+00,1.16e+00) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (4.2,1.1) \\
(10, 15, 2.0) & 0.8 & 0.8  & 0.6 & (1.35e+00,5.96e-02) & (1.35e+00,5.96e-02) & (1.20e+00,3.16e-02) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (6.7,0.5) \\
(20, 15, 2.0) & 0.4 & 0.4  & 1.0 & (1.24e+00,1.37e-01) & (1.24e+00,1.37e-01) & (1.10e+00,1.38e-01) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (8.0,1.1) \\
(30, 15, 2.0) & 0.6 & 0.4  & 1.0 & (2.71e+00,1.93e+00) & (1.35e+00,3.75e-02) & (1.26e+00,9.35e-02) & (2.3,1.2) & \tbcolor\bf (1.5,0.5) & (7.8,1.2) \\
(5, 20, 2.0) & 1.0 & 1.0  & 0.4 & (1.33e+00,1.54e-01) & (1.33e+00,1.54e-01) & (1.32e+00,1.44e-01) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (6.0,0.0) \\
(10, 20, 2.0) & 0.8 & 0.8  & 1.0 & (1.27e+00,1.08e-01) & (1.30e+00,1.03e-01) & (1.18e+00,1.64e-01) & \tbcolor\bf (1.8,0.4) & \tbcolor\bf (1.8,0.4) & (7.4,1.4) \\
(20, 20, 2.0) & 1.0 & 1.0  & 1.0 & (1.32e+00,5.54e-02) & (1.32e+00,5.54e-02) & (1.30e+00,8.38e-02) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (7.6,0.5) \\
(30, 20, 2.0) & 0.8 & 0.8  & 1.0 & (1.30e+00,1.19e-01) & (1.30e+00,1.19e-01) & (1.32e+00,8.85e-02) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (6.8,1.2) \\
(5, 50, 2.0) & 1.0 & 1.0  & 0.4 & (1.08e+00,1.71e-01) & (1.08e+00,1.71e-01) & (1.32e+00,3.29e-02) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (4.0,0.0) \\
(10, 50, 2.0) & 0.6 & 0.6  & 0.8 & (1.21e+00,1.31e-01) & (1.21e+00,1.31e-01) & (1.18e+00,1.54e-01) & \tbcolor\bf (1.7,0.5) & \tbcolor\bf (1.7,0.5) & (6.5,1.5) \\
(20, 50, 2.0) & 1.0 & 1.0  & 1.0 & (1.24e+00,9.01e-02) & (1.22e+00,6.12e-02) & (1.22e+00,1.52e-01) & (1.6,0.8) & \tbcolor\bf (1.4,0.5) & (8.6,1.7) \\
(30, 50, 2.0) & 1.0 & 1.0  & 1.0 & (1.26e+00,5.25e-02) & (1.26e+00,5.25e-02) & (1.23e+00,1.08e-01) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (6.8,1.3) \\
\end{tabular}


==> data/combined_table.tabular.tex <==
\begin{tabular}{ c | c c c | c c c | c c c }
\multirow{3}{*}{$(|\Sigma|, |A_{\mathrm{in}}|, \mathtt{tol})$} & \multicolumn{3}{c|}{success rate} & \multicolumn{3}{c|}{RMSE} & \multicolumn{3}{c}{$|A_{\mathrm{out}}|$} \\ \cline{2-10} 
 & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$} & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$} & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$}\\ 
 & minimized & not minimized &  & minimized & not minimized &  & minimized & not minimized & \\ \hline 
(5, 10, 0.5) & 0.8 & 1.0  & 1.0 & (6.49e-01,3.07e-02) & (5.85e-01,7.20e-02) & (5.65e-01,6.82e-02) & \tbcolor\bf (11.0,2.1) & (19.6,4.1) & (17.9,2.5) \\
(10, 10, 0.5) & 0.6 & 1.0  & 1.0 & (6.45e-01,4.91e-02) & (5.97e-01,6.83e-02) & (5.95e-01,6.12e-02) & \tbcolor\bf (14.5,1.7) & (31.3,7.3) & (22.0,3.6) \\
(20, 10, 0.5) & 0.3 & 1.0  & 1.0 & (5.86e-01,1.00e-01) & (4.75e-01,1.11e-01) & (6.30e-01,5.32e-02) & \tbcolor\bf (15.7,1.2) & (45.0,6.9) & (28.6,4.3) \\
(30, 10, 0.5) & 0.6 & 1.0  & 1.0 & (6.27e-01,5.93e-02) & (5.00e-01,6.33e-02) & (6.33e-01,3.41e-02) & \tbcolor\bf (16.3,4.3) & (56.1,12.1) & (31.2,3.0) \\
(5, 15, 0.5) & 0.9 & 0.9  & 1.0 & (6.68e-01,7.41e-02) & (5.81e-01,5.88e-02) & (5.63e-01,7.24e-02) & \tbcolor\bf (17.0,3.1) & (29.1,6.9) & (22.0,3.7) \\
(10, 15, 0.5) & 0.8 & 1.0  & 1.0 & (6.73e-01,4.43e-02) & (5.84e-01,6.64e-02) & (6.26e-01,4.63e-02) & \tbcolor\bf (28.4,5.7) & (61.4,7.9) & (36.9,6.4) \\
(20, 15, 0.5) & 0.7 & 1.0  & 1.0 & (6.42e-01,6.59e-02) & (5.35e-01,4.09e-02) & (6.48e-01,4.89e-02) & \tbcolor\bf (35.0,5.5) & (108.9,16.0) & (51.5,10.4) \\
(30, 15, 0.5) & 0.3 & 0.3  & 1.0 & (6.14e-01,5.17e-02) & (4.52e-01,3.12e-02) & (6.60e-01,3.35e-02) & \tbcolor\bf (34.7,4.5) & (114.7,6.6) & (55.3,9.9) \\
(5, 20, 0.5) & 0.4 & 0.9  & 1.0 & (6.10e-01,7.49e-02) & (5.97e-01,7.34e-02) & (6.09e-01,7.19e-02) & (29.5,3.2) & (46.6,8.9) & \tbcolor\bf (27.7,3.1) \\
(10, 20, 0.5) & 0.7 & 0.9  & 1.0 & (6.68e-01,3.49e-02) & (5.71e-01,4.07e-02) & (6.40e-01,3.40e-02) & \tbcolor\bf (47.1,5.4) & (117.9,17.7) & (48.9,10.1) \\
(20, 20, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.66e-01,2.75e-02) & N/A & N/A & \tbcolor\bf (68.4,17.2) \\
(30, 20, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.70e-01,3.47e-02) & N/A & N/A & \tbcolor\bf (88.2,25.9) \\
(5, 50, 0.5) & 0.2 & 0.2  & 1.0 & (5.80e-01,1.97e-02) & (5.66e-01,9.04e-03) & (6.67e-01,4.06e-02) & (90.0,1.0) & (164.5,3.5) & \tbcolor\bf (65.7,23.5) \\
(10, 50, 0.5) & 0.2 & 0.0  & 0.6 & (1.07e+01,2.53e+00) & N/A & (7.47e-01,1.74e-01) & \tbcolor\bf (1.0,0.0) & N/A & (95.5,20.6) \\
(20, 50, 0.5) & 0.0 & 0.0  & 0.0 & N/A & N/A & N/A & N/A & N/A & N/A \\
(30, 50, 0.5) & 0.0 & 0.1  & 0.0 & N/A & (8.98e+00,0.00e+00) & N/A & N/A & \tbcolor\bf (1.0,0.0) & N/A \\
(5, 10, 1.0) & 0.2 & 0.2  & 1.0 & (8.94e-01,4.64e-02) & (9.95e-01,2.20e-03) & (8.57e-01,1.05e-01) & \tbcolor\bf (3.5,0.5) & (5.5,2.5) & (9.9,1.3) \\
(10, 10, 1.0) & 0.4 & 0.7  & 1.0 & (1.19e+00,4.78e-01) & (9.45e-01,8.72e-02) & (8.70e-01,7.64e-02) & \tbcolor\bf (8.2,0.8) & (9.7,2.9) & (12.0,1.7) \\
(20, 10, 1.0) & 0.7 & 1.0  & 1.0 & (9.18e-01,4.68e-02) & (8.80e-01,4.08e-02) & (8.76e-01,8.62e-02) & \tbcolor\bf (9.3,0.7) & (12.3,3.7) & (13.6,2.6) \\
(30, 10, 1.0) & 0.8 & 0.9  & 1.0 & (8.89e-01,5.39e-02) & (8.88e-01,1.29e-01) & (7.99e-01,5.87e-02) & \tbcolor\bf (9.8,0.4) & (12.3,2.7) & (14.9,1.6) \\
(5, 15, 1.0) & 0.4 & 0.8  & 1.0 & (9.21e-01,4.52e-02) & (9.31e-01,6.90e-02) & (8.18e-01,1.30e-01) & \tbcolor\bf (2.2,0.4) & (5.2,2.4) & (10.1,2.2) \\
(10, 15, 1.0) & 0.4 & 0.7  & 1.0 & (9.43e-01,7.34e-02) & (1.07e+00,1.84e-01) & (8.60e-01,8.27e-02) & \tbcolor\bf (12.8,2.3) & (14.9,7.5) & (14.9,3.1) \\
(20, 15, 1.0) & 0.6 & 0.9  & 1.0 & (9.30e-01,5.17e-02) & (8.77e-01,7.46e-02) & (8.57e-01,7.11e-02) & \tbcolor\bf (15.0,0.6) & (20.7,5.8) & (18.1,2.9) \\
(30, 15, 1.0) & 0.7 & 0.9  & 1.0 & (9.23e-01,4.66e-02) & (9.52e-01,5.18e-02) & (8.89e-01,7.65e-02) & \tbcolor\bf (15.3,0.5) & (22.1,4.4) & (19.2,2.6) \\
(5, 20, 1.0) & 0.4 & 0.5  & 1.0 & (9.61e-01,1.22e-02) & (9.41e-01,6.14e-02) & (8.22e-01,8.86e-02) & (5.0,4.7) & \tbcolor\bf (4.2,2.6) & (12.8,1.9) \\
(10, 20, 1.0) & 0.5 & 0.5  & 1.0 & (9.79e-01,3.83e-02) & (9.42e-01,6.90e-02) & (9.13e-01,1.15e-01) & (17.0,4.0) & (21.0,5.8) & \tbcolor\bf (15.8,2.5) \\
(20, 20, 1.0) & 0.5 & 0.9  & 1.0 & (9.67e-01,4.61e-02) & (9.49e-01,5.81e-02) & (8.98e-01,3.87e-02) & \tbcolor\bf (17.0,5.1) & (25.4,9.6) & (22.2,4.6) \\
(30, 20, 1.0) & 0.5 & 0.9  & 1.0 & (9.20e-01,5.74e-02) & (9.28e-01,7.19e-02) & (9.40e-01,5.09e-02) & \tbcolor\bf (20.4,1.0) & (37.3,12.0) & (24.8,6.0) \\
(5, 50, 1.0) & 0.3 & 0.6  & 1.0 & (9.36e-01,6.51e-02) & (9.28e-01,8.52e-02) & (8.68e-01,7.79e-02) & \tbcolor\bf (3.7,1.2) & (9.3,9.1) & (18.5,6.5) \\
(10, 50, 1.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (9.31e-01,2.76e-02) & N/A & N/A & \tbcolor\bf (33.1,17.4) \\
(20, 50, 1.0) & 0.1 & 0.4  & 1.0 & (9.30e-01,0.00e+00) & (9.17e-01,4.48e-02) & (9.07e-01,8.39e-02) & \tbcolor\bf (43.0,0.0) & (50.2,25.2) & (49.4,25.1) \\
(30, 50, 1.0) & 0.0 & 0.5  & 1.0 & N/A & (2.49e+00,3.24e+00) & (9.22e-01,6.95e-02) & N/A & \tbcolor\bf (48.4,36.1) & (49.7,27.9) \\
(5, 10, 2.0) & 0.4 & 0.2  & 1.0 & (2.90e+00,2.83e+00) & (1.20e+00,6.81e-02) & (2.65e+00,2.41e+00) & (1.5,0.5) & \tbcolor\bf (1.0,0.0) & (6.0,1.6) \\
(10, 10, 2.0) & 0.4 & 0.4  & 0.7 & (1.27e+00,5.07e-02) & (1.27e+00,5.07e-02) & (1.57e+00,8.94e-01) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (6.0,1.7) \\
(20, 10, 2.0) & 0.1 & 0.1  & 1.0 & (1.25e+00,0.00e+00) & (1.25e+00,0.00e+00) & (1.20e+00,1.60e-01) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (8.0,1.5) \\
(30, 10, 2.0) & 0.4 & 0.3  & 1.0 & (1.34e+00,1.87e-02) & (1.34e+00,2.09e-02) & (1.22e+00,8.17e-02) & (1.8,0.4) & \tbcolor\bf (1.7,0.5) & (7.2,0.9) \\
(5, 15, 2.0) & 0.6 & 0.6  & 0.9 & (1.24e+00,1.49e-01) & (1.24e+00,1.49e-01) & (2.43e+00,1.18e+00) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (4.9,1.1) \\
(10, 15, 2.0) & 0.6 & 0.6  & 0.8 & (1.35e+00,4.95e-02) & (1.35e+00,4.95e-02) & (1.21e+00,1.12e-01) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (7.6,1.2) \\
(20, 15, 2.0) & 0.3 & 0.3  & 1.0 & (1.29e+00,1.39e-01) & (1.29e+00,1.39e-01) & (1.18e+00,1.40e-01) & \tbcolor\bf (1.3,0.5) & \tbcolor\bf (1.3,0.5) & (8.5,1.2) \\
(30, 15, 2.0) & 0.3 & 0.2  & 1.0 & (2.71e+00,1.93e+00) & (1.35e+00,3.75e-02) & (1.30e+00,9.24e-02) & (2.3,1.2) & \tbcolor\bf (1.5,0.5) & (8.3,1.5) \\
(5, 20, 2.0) & 0.7 & 0.7  & 0.7 & (1.31e+00,1.56e-01) & (1.31e+00,1.56e-01) & (1.32e+00,1.29e-01) & \tbcolor\bf (1.4,0.5) & \tbcolor\bf (1.4,0.5) & (6.9,1.2) \\
(10, 20, 2.0) & 0.5 & 0.5  & 1.0 & (1.29e+00,1.13e-01) & (1.32e+00,1.02e-01) & (1.23e+00,1.49e-01) & \tbcolor\bf (1.8,0.4) & \tbcolor\bf (1.8,0.4) & (9.4,2.5) \\
(20, 20, 2.0) & 0.5 & 0.5  & 1.0 & (1.32e+00,5.54e-02) & (1.32e+00,5.54e-02) & (1.33e+00,8.90e-02) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (8.9,1.9) \\
(30, 20, 2.0) & 0.4 & 0.4  & 1.0 & (1.30e+00,1.19e-01) & (1.30e+00,1.19e-01) & (1.33e+00,6.93e-02) & \tbcolor\bf (1.2,0.4) & \tbcolor\bf (1.2,0.4) & (8.3,1.9) \\
(5, 50, 2.0) & 0.6 & 0.6  & 0.7 & (1.13e+00,1.96e-01) & (1.10e+00,1.66e-01) & (1.23e+00,1.38e-01) & \tbcolor\bf (1.5,1.1) & \tbcolor\bf (1.5,1.1) & (7.6,2.4) \\
(10, 50, 2.0) & 0.4 & 0.4  & 0.9 & (1.25e+00,1.33e-01) & (1.25e+00,1.33e-01) & (1.23e+00,1.27e-01) & \tbcolor\bf (1.8,0.4) & \tbcolor\bf (1.8,0.4) & (9.0,3.1) \\
(20, 50, 2.0) & 0.5 & 0.5  & 1.0 & (1.24e+00,9.01e-02) & (1.22e+00,6.12e-02) & (1.28e+00,1.27e-01) & (1.6,0.8) & \tbcolor\bf (1.4,0.5) & (11.5,3.3) \\
(30, 50, 2.0) & 0.5 & 0.6  & 1.0 & (1.26e+00,5.25e-02) & (1.88e+00,1.40e+00) & (1.27e+00,1.04e-01) & \tbcolor\bf (1.2,0.4) & (5.5,9.6) & (10.7,4.8) \\
\end{tabular}


==> data/gamma_table.tabular.tex <==
\begin{tabular}{ c | c c c | c c c | c c c }
\multirow{3}{*}{$(|\Sigma|, |A_{\mathrm{in}}|, \mathtt{tol})$} & \multicolumn{3}{c|}{succ. rate} & \multicolumn{3}{c|}{RMSE} & \multicolumn{3}{c}{$|A_{\mathrm{out}}|$} \\ \cline{2-10} 
 & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$} & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$} & $\rmax$ & $\rmax$ & \multirow{2}{*}{$\real$}\\ 
 & minimized & not minimized &  & minimized & not minimized &  & minimized & not minimized & \\ \hline 
(5, 10, 0.5) & 0.6 & 1.0  & 1.0 & (6.60e-01,8.65e-03) & (5.86e-01,6.72e-02) & (5.94e-01,5.45e-02) & \tbcolor\bf (11.7,2.5) & (21.4,4.7) & (17.2,2.3) \\
(10, 10, 0.5) & 0.6 & 1.0  & 1.0 & (6.57e-01,2.62e-02) & (5.56e-01,5.71e-02) & (5.76e-01,7.48e-02) & \tbcolor\bf (13.3,1.2) & (30.4,5.8) & (22.0,4.3) \\
(20, 10, 0.5) & 0.4 & 1.0  & 1.0 & (5.18e-01,3.30e-02) & (4.11e-01,7.51e-02) & (6.48e-01,4.93e-02) & \tbcolor\bf (15.0,1.0) & (41.8,5.3) & (31.4,3.3) \\
(30, 10, 0.5) & 0.8 & 1.0  & 1.0 & (6.16e-01,6.72e-02) & (4.65e-01,4.26e-02) & (6.35e-01,3.57e-02) & \tbcolor\bf (14.0,1.9) & (46.0,4.2) & (33.2,2.2) \\
(5, 15, 0.5) & 0.8 & 0.8  & 1.0 & (6.63e-01,7.13e-02) & (5.70e-01,4.69e-02) & (5.59e-01,7.44e-02) & \tbcolor\bf (19.2,1.5) & (33.0,1.6) & (25.2,2.2) \\
(10, 15, 0.5) & 0.8 & 1.0  & 1.0 & (6.64e-01,4.67e-02) & (5.74e-01,6.58e-02) & (6.42e-01,1.92e-02) & \tbcolor\bf (28.2,4.8) & (59.8,3.8) & (42.6,2.3) \\
(20, 15, 0.5) & 1.0 & 1.0  & 1.0 & (6.12e-01,5.28e-02) & (5.16e-01,4.47e-02) & (6.72e-01,3.83e-02) & \tbcolor\bf (32.6,4.6) & (105.4,18.9) & (60.4,4.1) \\
(30, 15, 0.5) & 0.6 & 0.6  & 1.0 & (6.14e-01,5.17e-02) & (4.52e-01,3.12e-02) & (6.77e-01,2.12e-02) & \tbcolor\bf (34.7,4.5) & (114.7,6.6) & (63.6,7.2) \\
(5, 20, 0.5) & 0.2 & 0.8  & 1.0 & (5.02e-01,0.00e+00) & (5.91e-01,5.54e-02) & (6.56e-01,5.55e-02) & \tbcolor\bf (29.0,0.0) & (51.2,7.9) & (29.4,2.2) \\
(10, 20, 0.5) & 0.6 & 0.8  & 1.0 & (6.94e-01,2.82e-02) & (5.45e-01,1.49e-02) & (6.53e-01,2.45e-02) & \tbcolor\bf (45.0,5.0) & (128.0,17.2) & (58.4,4.0) \\
(20, 20, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.86e-01,2.24e-02) & N/A & N/A & \tbcolor\bf (83.2,9.2) \\
(30, 20, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.98e-01,1.40e-02) & N/A & N/A & \tbcolor\bf (113.0,4.1) \\
(5, 50, 0.5) & 0.0 & 0.0  & 1.0 & N/A & N/A & (6.64e-01,4.14e-02) & N/A & N/A & \tbcolor\bf (86.6,8.5) \\
(10, 50, 0.5) & 0.0 & 0.0  & 0.2 & N/A & N/A & (1.13e+00,0.00e+00) & N/A & N/A & \tbcolor\bf (137.0,0.0) \\
(20, 50, 0.5) & 0.0 & 0.0  & 0.0 & N/A & N/A & N/A & N/A & N/A & N/A \\
(30, 50, 0.5) & 0.0 & 0.2  & 0.0 & N/A & (8.98e+00,0.00e+00) & N/A & N/A & \tbcolor\bf (1.0,0.0) & N/A \\
(5, 10, 1.0) & 0.4 & 0.2  & 1.0 & (8.94e-01,4.64e-02) & (9.93e-01,0.00e+00) & (8.27e-01,6.98e-02) & (3.5,0.5) & \tbcolor\bf (3.0,0.0) & (9.8,1.5) \\
(10, 10, 1.0) & 0.4 & 0.6  & 1.0 & (1.48e+00,5.25e-01) & (9.63e-01,5.25e-02) & (9.03e-01,7.55e-02) & \tbcolor\bf (8.0,1.0) & (10.3,1.2) & (11.4,1.4) \\
(20, 10, 1.0) & 0.6 & 1.0  & 1.0 & (9.08e-01,4.48e-02) & (8.58e-01,2.95e-02) & (9.08e-01,4.10e-02) & \tbcolor\bf (9.7,0.5) & (15.0,2.1) & (14.4,1.0) \\
(30, 10, 1.0) & 1.0 & 0.8  & 1.0 & (8.87e-01,6.37e-02) & (8.10e-01,1.26e-01) & (7.99e-01,6.52e-02) & \tbcolor\bf (9.8,0.4) & (14.2,2.5) & (15.2,2.1) \\
(5, 15, 1.0) & 0.2 & 0.6  & 1.0 & (9.96e-01,0.00e+00) & (9.67e-01,2.07e-02) & (8.18e-01,1.13e-01) & \tbcolor\bf (2.0,0.0) & (5.3,2.4) & (11.0,2.1) \\
(10, 15, 1.0) & 0.2 & 0.8  & 1.0 & (9.89e-01,0.00e+00) & (1.13e+00,2.30e-01) & (8.79e-01,4.17e-02) & \tbcolor\bf (15.0,0.0) & (21.0,2.1) & (17.6,1.2) \\
(20, 15, 1.0) & 0.4 & 0.8  & 1.0 & (9.50e-01,3.36e-02) & (8.89e-01,4.43e-02) & (8.75e-01,8.85e-02) & \tbcolor\bf (15.0,0.0) & (26.0,2.9) & (20.4,2.5) \\
(30, 15, 1.0) & 1.0 & 1.0  & 1.0 & (9.32e-01,4.85e-02) & (9.74e-01,4.70e-02) & (9.11e-01,6.51e-02) & \tbcolor\bf (15.2,0.4) & (25.0,3.4) & (21.0,2.0) \\
(5, 20, 1.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (8.14e-01,1.11e-01) & N/A & N/A & \tbcolor\bf (14.2,1.2) \\
(10, 20, 1.0) & 0.4 & 0.4  & 1.0 & (9.91e-01,2.95e-02) & (9.46e-01,4.26e-02) & (9.73e-01,6.66e-02) & (19.5,0.5) & (27.5,1.5) & \tbcolor\bf (18.0,0.6) \\
(20, 20, 1.0) & 0.2 & 1.0  & 1.0 & (9.59e-01,0.00e+00) & (9.18e-01,3.40e-02) & (8.83e-01,4.43e-02) & \tbcolor\bf (20.0,0.0) & (32.2,2.9) & (26.0,3.2) \\
(30, 20, 1.0) & 0.4 & 0.8  & 1.0 & (8.72e-01,1.47e-02) & (8.82e-01,6.49e-02) & (9.49e-01,4.65e-02) & \tbcolor\bf (21.0,1.0) & (48.8,6.9) & (30.0,3.3) \\
(5, 50, 1.0) & 0.0 & 0.2  & 1.0 & N/A & (1.03e+00,0.00e+00) & (8.88e-01,4.41e-02) & N/A & (28.0,0.0) & \tbcolor\bf (24.0,3.8) \\
(10, 50, 1.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (9.30e-01,3.12e-02) & N/A & N/A & \tbcolor\bf (50.2,4.4) \\
(20, 50, 1.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (9.54e-01,1.67e-02) & N/A & N/A & \tbcolor\bf (73.8,6.4) \\
(30, 50, 1.0) & 0.0 & 0.2  & 1.0 & N/A & (8.98e+00,0.00e+00) & (9.58e-01,4.68e-02) & N/A & \tbcolor\bf (1.0,0.0) & (77.2,3.2) \\
(5, 10, 2.0) & 0.4 & 0.2  & 1.0 & (4.47e+00,3.34e+00) & (1.13e+00,0.00e+00) & (1.81e+00,9.14e-01) & (1.5,0.5) & \tbcolor\bf (1.0,0.0) & (6.2,1.2) \\
(10, 10, 2.0) & 0.2 & 0.2  & 0.8 & (1.28e+00,0.00e+00) & (1.28e+00,0.00e+00) & (1.88e+00,1.06e+00) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (6.2,2.2) \\
(20, 10, 2.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (1.20e+00,1.93e-01) & N/A & N/A & \tbcolor\bf (8.6,0.8) \\
(30, 10, 2.0) & 0.2 & 0.2  & 1.0 & (1.36e+00,0.00e+00) & (1.36e+00,0.00e+00) & (1.18e+00,6.40e-02) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (7.8,0.7) \\
(5, 15, 2.0) & 0.4 & 0.4  & 1.0 & (1.37e+00,1.03e-01) & (1.37e+00,1.03e-01) & (2.08e+00,1.07e+00) & \tbcolor\bf (1.0,0.0) & \tbcolor\bf (1.0,0.0) & (5.4,0.8) \\
(10, 15, 2.0) & 0.4 & 0.4  & 1.0 & (1.34e+00,1.05e-02) & (1.34e+00,1.05e-02) & (1.22e+00,1.39e-01) & \tbcolor\bf (1.5,0.5) & \tbcolor\bf (1.5,0.5) & (8.2,1.2) \\
(20, 15, 2.0) & 0.2 & 0.2  & 1.0 & (1.41e+00,0.00e+00) & (1.41e+00,0.00e+00) & (1.26e+00,9.15e-02) & \tbcolor\bf (2.0,0.0) & \tbcolor\bf (2.0,0.0) & (9.0,1.1) \\
(30, 15, 2.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (1.33e+00,7.44e-02) & N/A & N/A & \tbcolor\bf (8.8,1.6) \\
(5, 20, 2.0) & 0.4 & 0.4  & 1.0 & (1.25e+00,1.50e-01) & (1.25e+00,1.50e-01) & (1.32e+00,1.23e-01) & \tbcolor\bf (2.0,0.0) & \tbcolor\bf (2.0,0.0) & (7.2,1.3) \\
(10, 20, 2.0) & 0.2 & 0.2  & 1.0 & (1.41e+00,0.00e+00) & (1.41e+00,0.00e+00) & (1.27e+00,1.16e-01) & \tbcolor\bf (2.0,0.0) & \tbcolor\bf (2.0,0.0) & (11.4,1.5) \\
(20, 20, 2.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (1.36e+00,8.34e-02) & N/A & N/A & \tbcolor\bf (10.2,1.8) \\
(30, 20, 2.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (1.33e+00,4.15e-02) & N/A & N/A & \tbcolor\bf (9.8,1.2) \\
(5, 50, 2.0) & 0.2 & 0.2  & 1.0 & (1.40e+00,0.00e+00) & (1.23e+00,0.00e+00) & (1.19e+00,1.46e-01) & \tbcolor\bf (4.0,0.0) & \tbcolor\bf (4.0,0.0) & (9.0,1.1) \\
(10, 50, 2.0) & 0.2 & 0.2  & 1.0 & (1.37e+00,0.00e+00) & (1.37e+00,0.00e+00) & (1.26e+00,8.19e-02) & \tbcolor\bf (2.0,0.0) & \tbcolor\bf (2.0,0.0) & (11.0,2.6) \\
(20, 50, 2.0) & 0.0 & 0.0  & 1.0 & N/A & N/A & (1.33e+00,5.62e-02) & N/A & N/A & \tbcolor\bf (14.4,1.2) \\
(30, 50, 2.0) & 0.0 & 0.2  & 1.0 & N/A & (5.02e+00,0.00e+00) & (1.30e+00,8.64e-02) & N/A & (27.0,0.0) & \tbcolor\bf (14.6,3.7) \\
\end{tabular}


==> data/res_combined_smash_asize_insize.tabular.tex <==
\begin{tabular}{ c | c c c }
tol. & $\rmax$ (minimized) & $\rmax$ (not minimized) & $\real$ \\ \hline
0.5 & (6.44e-01,6.32e-02) & (5.54e-01,8.15e-02) & (6.30e-01,6.14e-02)  \\
1.0 & (9.29e-01,5.78e-02) & (9.25e-01,7.93e-02) & (8.77e-01,9.07e-02)  \\
2.0 & (1.27e+00,1.28e-01) & (1.27e+00,1.27e-01) & (1.44e+00,8.51e-01)  \\
\end{tabular}


==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

\def\gnuplot@output@ps{ps} % required for comparison in \gprawimage

\expandafter\def\csname gnuplot@select@driver@pgfsys-dvi.def\endcsname     {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfm.def\endcsname {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfmx.def\endcsname{pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvips.def\endcsname   {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-pdftex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-luatex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-tex4ht.def\endcsname  {html}
\expandafter\def\csname gnuplot@select@driver@pgfsys-textures.def\endcsname{ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-vtex.def\endcsname    {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-xetex.def\endcsname   {pdf}

\ifcsname gnuplot@select@driver@\pgfsysdriver\endcsname
  \edef\gnuplot@output@mode{\csname gnuplot@select@driver@\pgfsysdriver\endcsname}
\else
  \errmessage{The driver \pgfsysdriver\space is not supported by gnuplot-lua-tikz}%
\fi

\ifcsname PackageWarning\endcsname
  \let\gnuplot@packagewarning\PackageWarning
\else
  \def\gnuplot@packagewarning#1#2{\immediate\write-1{Package #1 Warning: #2}}
\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
  \gnuplot@packagewarning{gnuplot-lua-tikz}{%
    \noexpand\gp@rawimage is not implemented for \gnuplot@output@mode\space output.%
  }%
}

% Select \gp@rawimage depending on the output mode
\expandafter\let\expandafter\gp@rawimage\csname gp@rawimage@\gnuplot@output@mode\endcsname

\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{%
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext{%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
  \else
    \ifx\gnuplot@output@mode\gnuplot@output@ps
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}%
    \fi
  \fi
}

%
% gnuplottex compatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
% 3-parameter variant gp3point passes style options as well as point type and coordinates
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}
\def\gp3point#1#2#3{%
  \path[solid#2] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#3};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}%
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }%
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex,line width=0pt}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex,line width=0pt}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex,line width=0pt}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds,fit}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode

\endinput


==> t-gnuplot-lua-tikz.tex <==
%%
%%  ConTeXt wrapper for gnuplot-tikz style file
%%
\usemodule[tikz]

\usetikzlibrary[arrows,patterns,plotmarks,backgrounds,fit]

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\endinput

